Small-signal stability in inverter-dominated grids: exploring the role of gains, line dynamics, and operating conditions

In a power grid with growing penetrations of renewable energy sources, inverters play a larger role in the dynamic interactions among network components. However, much is yet to be studied regarding inverter-dominated grid stability. This has initiated a re-examination of long-established assumptions made when conducting power systems studies. In this work we study the small-signal stability characteristics of a power system comprised of inverter and synchronous machine sources, and consider the effect of inverter control gains, transmission line dynamics, and network operating conditions. We utilize PowerSimulationsDynamics.jl to perform this study on the IEEE WSCC 9 Bus test system. We vary inverter parameters across reported ranges in the literature, we consider three transmission line models of varying fidelity, and compare results across different operating conditions. We find that line dynamics are generally important for correctly assessing small-signal stability in networks with large penetrations of grid-following converters, and that gain tuning in these networks should utilize high fidelity line models.

==> extra.tex <==
% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccc}
%         \hline 
%         \textbf{Load} & \textbf{P} & \textbf{Q} \\ \hline 
%         Bus 5 Load & 1.25 & 0.5 \\
%         Bus 6 Load & 0.9 & 0.3 \\
%         Bus 8 Load &  1.0 & 0.35 \\
%         \hline 
%     \end{tabular}
%     \caption{9 bus loads}
%     \label{tab:9 bus loads}
% \end{table}
%
% \begin{table}[h]
%     \centering
%     \begin{tabular}{cc}
%         \hline 
%         \textbf{Line} & \textbf{Length (km)} \\ \hline 
%         Bus 5-4 & 90 \\
%         Bus 7-8 & 80 \\
%         Bus 6-4 & 100 \\
%         Bus 7-5 & 170 \\
%         Bus 8-9 & 110 \\
%         \hline 
%     \end{tabular}
%     \caption{9 bus loads}
%     \label{tab:9bus_line_lengths}
% \end{table}
%


% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccccc}
%         \hline 
%         \textbf{Parameter} & \textbf{Symbol} & \textbf{Value} & Units & Ref \\ \hline \hline 
%         Active power control - P gain & $k_{pp}$ & 0.0059 & & \\
%         Active power control - I gain & $k_{ip}$& 7.36 & &\\
%         Active power control P ref & $P_{ref}$ & 0.5 & & \\
%         Active power control filter freq & $\omega_z$  & 1000 & ? & \\
%         Reactive power control - P gain & $k_{pq}$& 0.0059 & &\\
%         Reactive power control - I gain & $k_{iq} $& 7.36 & &\\ 
%         Reactive power control filter freq & $\omega_f$  & 1000 & ? & \\
%         Reactive power control V ref & $V_{ref}$ & 1.0 & ? & \\
%         Reactive power control Q ref & $Q_{ref}$ & 0.1 & ? & \\
%         Inner current control - P gain & $k_{pc}$& 1.27 & &\\ 
%         Inner current control - I gain & $k_{ic}$& 14.3 & &\\ 
%         Inner current control - voltage FF gain & $k_{ffc}$& 0.0 & &\\ 
%         PLL: P gain & $k_{p,pll}$& 0.084 &  & \\
%         PLL: I gain & $k_{i,pll}$& 4.69 &  & \\
%         PLL: low pass filter freq & $\omega_{lp}$& 500 & rad/s & \\
%         \hline 
%     \end{tabular}
%     \caption{GFL and SM parameters}
%     \label{tab:GFL_SM_params}
% \end{table}



% \begin{figure*}[tb]
%  \begin{subfigure}[t]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{figures/_kd.png}
%     \caption{$k_d$}
%         \label{fig:kd}
%   \end{subfigure}
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/_kpc.png}
%         \caption{$k_{pc}$}
%         \label{fig:kpc}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/_kic.png}
%         \caption{$k_{ic}$}
%         \label{fig:kic}
%     \end{subfigure}
%     \label{fig:ccccc}
%     \vfill
% \begin{subfigure}[t]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{figures/_kq.png}
%     \caption{$k_q$}
%         \label{fig:kq}
%   \end{subfigure}
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/_kpv.png}
%         \caption{$k_{pv}$}
%         \label{fig:kpv}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/_kiv.png}
%         \caption{$k_{iv}$}
%         \label{fig:kiv}
%     \end{subfigure}
%     \label{fig:ccccc}
%     \vfill
% \begin{subfigure}[t]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{figures/_gfm_eta.png}
%         \caption{$\eta_{gfm}$}
%         \label{fig:gfm_eta}
%   \end{subfigure}
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/_gfl_eta.png}
%         \caption{$\eta_{gfl}$}
%         \label{fig:gfl_eta}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/_load_scale.png}
%         \caption{Load scale}
%         \label{fig:load_scale}
%     \end{subfigure}
%     \caption{Results with D'Arco inverter parameters \cite{d2015virtual}, with outer loop PI gains chosen to maintain consistency with timescale separation of inner and outer loops. 100 samples. Line scale=1.0.}
%     \label{fig:boxplots_nom}
% \end{figure*}



% \begin{figure*}[tb]
% \centering
%  \begin{subfigure}[t]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{figures/low_load_low_gfl_boxplot.png}
%     \caption{Low load, low GFL}
%         \label{fig:low_load_low_gfl}
%   \end{subfigure}
%     \begin{subfigure}[t]{0.4\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/low_load_high_gfl_boxplot.png}
%         \caption{Low load, high GFL}
%         \label{fig:low_load_high_gfl}
%     \end{subfigure}
%         \vfill
%     \begin{subfigure}[t]{0.4\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/nom_load_low_gfl_boxplot.png}
%         \caption{Nominal load, low GFL}
%         \label{fig:nominal_load_low_gfl}
%     \end{subfigure}
% \begin{subfigure}[t]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{figures/nom_load_high_gfl_boxplot.png}
%         \caption{Nominal load, high GFL}
%         \label{fig:nominal_load_high_gfl}
%     \end{subfigure}
%     \caption{For system with line length=3.0. Low load is \textit{load scale}=0.5, nominal load is \textit{load scale}=1.0, Low GFL is $\eta_{gfl}=0.08$ (i.e., 8\% of generation), High GFL is $\eta_{gfl}=0.32$ (i.e., 32\% of generation)- only 50 samples. } 
%     \label{fig:2x2_cases}
% \end{figure*}
